Tag loss models for capture-recapture data without double tagging

Standard capture-recapture (CR) models assume that marked individuals do not lose their tags during the sampling period. When this assumption is violated, the estimates of model parameters can be biased. Existing tag-loss models generally rely on double-tagging all or a subset of captured individuals, permanent marks, or auxiliary information on tag retention. However, double-tagging and permanent marking may be impractical, and reliable auxiliary information may be unavailable or difficult to obtain in many situations. In this paper, we develop a novel latent multinomial modelling framework for analysis of CR data with tag loss, without requiring double-tagging or permanent marking. The proposed model framework applies to both closed-population and open-population Cormack-Jolly-Seber (CJS) settings. Through simulation studies, we demonstrate that key model parameters can be reliably estimated in both settings. We illustrate the application of the method using a dataset from a long-term study on elephant seals. The results suggest that robust inference on tag loss and demographic parameters can be achieved without double tagging, thereby avoiding logistical challenges and broadening the framework's applicability to a wider range of studies.

==> supplementary_material.tex <==


\section{Supplementary Material}\label{supp_mat}

